Entanglements

Robertson and Seymour constructed for every graph $G$ a tree-decomposition that efficiently distinguishes all the tangles in $G$. While all previous constructions of these decompositions are either iterative in nature or not canonical, we give an explicit one-step construction that is canonical. The key ingredient is an axiomatisation of 'local properties' of tangles. Generalisations to locally finite graphs and matroids are also discussed.

==> minimalJ.tex <==
% This is my basic toolkit; things I will always want.

% First, some packages:
\usepackage{epsfig}
\usepackage{graphicx}
\usepackage{amsbsy}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{textcomp}
\usepackage{hyperref}
\usepackage{aliascnt}

% Then, some commands I'll need:
% Nicked  from Leinster:
\newcommand{\mcm}[3]{\newcommand{#1}[#2]{{\ensuremath{#3}}}} 

\mcm{\tuple}{1}{\langle #1 \rangle}
\mcm{\name}{1}{\ulcorner #1 \urcorner}
\mcm{\Nbb}{0}{\mathbb{N}}
\mcm{\Zbb}{0}{\mathbb{Z}}
\mcm{\Rbb}{0}{\mathbb{R}}
\mcm{\Cbb}{0}{\mathbb{C}}
\mcm{\Qbb}{0}{\mathbb{Q}}
\mcm{\Acal}{0}{\cal A}
\mcm{\Bcal}{0}{\cal B}
\mcm{\Ccal}{0}{\cal C}
\mcm{\Dcal}{0}{\cal D}
\mcm{\Ecal}{0}{\mathcal E}
\mcm{\Fcal}{0}{\cal F}
\mcm{\Gcal}{0}{\cal G}
\mcm{\Hcal}{0}{\cal H}
\mcm{\Ical}{0}{\cal I}
\mcm{\Jcal}{0}{\cal J}
\mcm{\Kcal}{0}{\cal K}
\mcm{\Lcal}{0}{\cal L}
\mcm{\Mcal}{0}{\cal M}
\mcm{\Ncal}{0}{\cal N}
\mcm{\Ocal}{0}{{\cal O}}
\mcm{\Pcal}{0}{{\cal P}}
\mcm{\Qcal}{0}{{\cal Q}}
\mcm{\Rcal}{0}{{\cal R}}
\mcm{\Scal}{0}{{\cal S}}
\mcm{\Tcal}{0}{{\mathcal T}}
\mcm{\Ucal}{0}{{\cal U}}
\mcm{\Vcal}{0}{{\mathcal V}}
\mcm{\Wcal}{0}{{\cal W}}
\mcm{\Xcal}{0}{{\cal X}}
\mcm{\Ycal}{0}{{\cal Y}}
\mcm{\Zcal}{0}{{\cal Z}}
\mcm{\Mfrak}{0}{\mathfrak M}
\newcommand{\easy}{\nobreak\hfill$\square$\medskip}
\newcommand{\contradiction}{\nobreak\hfill\textreferencemark\medskip}
\DeclareMathOperator{\Cl}{Cl}
\mcm{\restric}{0}{\upharpoonright}
\mcm{\upset}{0}{\uparrow}
\mcm{\onto}{0}{\twoheadrightarrow}
\mcm{\smallNbb}{0}{{\small \mathbb{N}}}
\DeclareMathOperator{\preop}{op}
\mcm{\op}{0}{^{\preop}}
\newcommand{\supth}{\textsuperscript{th}}
\newcommand{\supst}{\textsuperscript{st}}
\newcommand{\supnd}{\textsuperscript{nd}}
\newcommand{\itum}{\item[$\bullet$]}
\newcommand{\se}{\subseteq}
%I like this environment, which is one of Leinster's:
\newenvironment{centredpic}%
{\begin{array}{c}
\setlength{\unitlength}{1em}}%
{\end{array}}

%Finally, I'll want the following theorem structure:
\usepackage{amsthm}

\newcommand{\theoremize}[2]{\newaliascnt{#1}{thm} \newtheorem{#1}[#1]{#2} \aliascntresetthe{#1}}

\theoremstyle{plain}
\newtheorem{thm}{Theorem}[section]
\theoremize{lem}{Lemma}
\theoremize{skolem}{Skolem}
\theoremize{fact}{Fact}
\theoremize{sublem}{Sublemma}
\theoremize{claim}{Claim}
\theoremize{obs}{Observation}
\theoremize{prop}{Proposition}
\theoremize{cor}{Corollary}
\theoremize{que}{Question}
\theoremize{oque}{Open Question}
\theoremize{con}{Conjecture}

\theoremstyle{definition}
\theoremize{dfn}{Definition}
\newtheorem*{maindfn}{Definition}
\theoremize{rem}{Remark}
\theoremize{eg}{Example}
\theoremize{exercise}{Exercise}
\theoremstyle{plain}


\def\subsubsectionautorefname{Section}
\def\subsectionautorefname{Section}
\def\thmautorefname{Theorem}
\def\lemautorefname{Lemma}
\def\skolemautorefname{Skolem}
\def\factautorefname{Fact}
\def\sublemautorefname{Sublemma}
\def\claimautorefname{Claim}
\def\remautorefname{Remark}
\def\obsautorefname{Observation}
\def\propautorefname{Proposition}
\def\corautorefname{Corollary}
\def\queautorefname{Question}
\def\oqueautorefname{Open Question}
\def\conautorefname{Conjecture}
\def\dfnautorefname{Definition}
\def\egautorefname{Example}
\def\exerciseautorefname{Exercise}
\def\sectionautorefname{Section}
\def\figureautorefname{Figure}
\def\tableautorefname{Table}



\newcommand{\myref}[1]{\autoref{#1}~(\nameref{#1})}
